Implementing Set-Theoretic Types

Set-theoretic types provide a rich type algebra that supports unrestricted unions, intersections, and negations, together with a decidable type constraint-solving algorithm known as tallying. These types are particularly well suited for typing dynamic languages, where functions often exhibit both generic and overloaded behavior. However, the complexity of their implementation has hindered their widespread adoption. In this paper, we introduce a modular representation for set-theoretic types and revisit the algorithms for subtyping and tallying. We compare our approach with the historical CDuce implementation and evaluate the performance impact of some optimizations and design choices.

==> timing.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(7920.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(100,657){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(100,903){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \csname LTb\endcsname%%
      \put(100,1150){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \csname LTb\endcsname%%
      \put(100,1396){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \csname LTb\endcsname%%
      \put(100,1643){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \csname LTb\endcsname%%
      \put(100,1889){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(100,2136){\makebox(0,0)[r]{\strut{}$1.2$}}%
      \csname LTb\endcsname%%
      \put(411,495){\rotatebox{45.00}{\makebox(0,0)[r]{\strut{}BDT}}}%
      \csname LTb\endcsname%%
      \put(621,495){\rotatebox{45.00}{\makebox(0,0)[r]{\strut{}SS$\star$}}}%
      \csname LTb\endcsname%%
      \put(831,495){\rotatebox{45.00}{\makebox(0,0)[r]{\strut{}HC}}}%
      \csname LTb\endcsname%%
      \put(1041,495){\rotatebox{45.00}{\makebox(0,0)[r]{\strut{}SS+HC}}}%
      \csname LTb\endcsname%%
      \put(1461,495){\rotatebox{45.00}{\makebox(0,0)[r]{\strut{}BDT}}}%
      \csname LTb\endcsname%%
      \put(1671,495){\rotatebox{45.00}{\makebox(0,0)[r]{\strut{}SS}}}%
      \csname LTb\endcsname%%
      \put(2143,495){\rotatebox{45.00}{\makebox(0,0)[r]{\strut{}SS}}}%
      \csname LTb\endcsname%%
      \put(2616,495){\rotatebox{45.00}{\makebox(0,0)[r]{\strut{}CDuce}}}%
      \csname LTb\endcsname%%
      \put(2826,495){\rotatebox{45.00}{\makebox(0,0)[r]{\strut{}BDT}}}%
      \csname LTb\endcsname%%
      \put(3036,495){\rotatebox{45.00}{\makebox(0,0)[r]{\strut{}SS$\star$}}}%
      \csname LTb\endcsname%%
      \put(3246,495){\rotatebox{45.00}{\makebox(0,0)[r]{\strut{}HC}}}%
      \csname LTb\endcsname%%
      \put(3456,495){\rotatebox{45.00}{\makebox(0,0)[r]{\strut{}SS+HC}}}%
      \csname LTb\endcsname%%
      \put(3875,495){\rotatebox{45.00}{\makebox(0,0)[r]{\strut{}BDT}}}%
      \csname LTb\endcsname%%
      \put(4085,495){\rotatebox{45.00}{\makebox(0,0)[r]{\strut{}SS}}}%
      \csname LTb\endcsname%%
      \put(4558,495){\rotatebox{45.00}{\makebox(0,0)[r]{\strut{}SS}}}%
      \csname LTb\endcsname%%
      \put(5030,495){\rotatebox{45.00}{\makebox(0,0)[r]{\strut{}CDuce}}}%
      \csname LTb\endcsname%%
      \put(5240,495){\rotatebox{45.00}{\makebox(0,0)[r]{\strut{}BDT}}}%
      \csname LTb\endcsname%%
      \put(5450,495){\rotatebox{45.00}{\makebox(0,0)[r]{\strut{}SS$\star$}}}%
      \csname LTb\endcsname%%
      \put(5660,495){\rotatebox{45.00}{\makebox(0,0)[r]{\strut{}HC}}}%
      \csname LTb\endcsname%%
      \put(5870,495){\rotatebox{45.00}{\makebox(0,0)[r]{\strut{}SS+HC}}}%
      \csname LTb\endcsname%%
      \put(6290,495){\rotatebox{45.00}{\makebox(0,0)[r]{\strut{}BDT}}}%
      \csname LTb\endcsname%%
      \put(6500,495){\rotatebox{45.00}{\makebox(0,0)[r]{\strut{}SS}}}%
      \csname LTb\endcsname%%
      \put(6973,495){\rotatebox{45.00}{\makebox(0,0)[r]{\strut{}SS}}}%
      \csname LTb\endcsname%%
      \put(7445,495){\rotatebox{45.00}{\makebox(0,0)[r]{\strut{}CDuce}}}%
      \csname LTb\endcsname%%
      \put(306,3121){\makebox(0,0)[l]{\strut{}Time (s)}}%
      \csname LTb\endcsname%%
      \put(1461,2819){\makebox(0,0){\strut{}Corpus A (872 instances)}}%
      \csname LTb\endcsname%%
      \put(726,2579){\rotatebox{30.00}{\makebox(0,0){\strut{}Type}}}%
      \put(726,2435){\rotatebox{30.00}{\makebox(0,0){\strut{}representation}}}%
      \csname LTb\endcsname%%
      \put(1566,2579){\rotatebox{30.00}{\makebox(0,0){\strut{}Naive}}}%
      \put(1566,2435){\rotatebox{30.00}{\makebox(0,0){\strut{} \texttt{is\_empty}}}}%
      \csname LTb\endcsname%%
      \put(2196,2579){\rotatebox{30.00}{\makebox(0,0){\strut{}Naive}}}%
      \put(2196,2435){\rotatebox{30.00}{\makebox(0,0){\strut{} \texttt{tally}}}}%
      \csname LTb\endcsname%%
      \put(2395,2136){\makebox(0,0){\strut{}8.609s}}%
      \csname LTb\endcsname%%
      \put(3875,2819){\makebox(0,0){\strut{}Corpus B (5514 instances)}}%
      \csname LTb\endcsname%%
      \put(3141,2579){\rotatebox{30.00}{\makebox(0,0){\strut{}Type}}}%
      \put(3141,2435){\rotatebox{30.00}{\makebox(0,0){\strut{}representation}}}%
      \csname LTb\endcsname%%
      \put(3980,2579){\rotatebox{30.00}{\makebox(0,0){\strut{}Naive}}}%
      \put(3980,2435){\rotatebox{30.00}{\makebox(0,0){\strut{} \texttt{is\_empty}}}}%
      \csname LTb\endcsname%%
      \put(4610,2579){\rotatebox{30.00}{\makebox(0,0){\strut{}Naive}}}%
      \put(4610,2435){\rotatebox{30.00}{\makebox(0,0){\strut{} \texttt{tally}}}}%
      \csname LTb\endcsname%%
      \put(6290,2819){\makebox(0,0){\strut{}Corpus C (2358 instances)}}%
      \csname LTb\endcsname%%
      \put(5555,2579){\rotatebox{30.00}{\makebox(0,0){\strut{}Type}}}%
      \put(5555,2435){\rotatebox{30.00}{\makebox(0,0){\strut{}representation}}}%
      \csname LTb\endcsname%%
      \put(6395,2579){\rotatebox{30.00}{\makebox(0,0){\strut{}Naive}}}%
      \put(6395,2435){\rotatebox{30.00}{\makebox(0,0){\strut{} \texttt{is\_empty}}}}%
      \csname LTb\endcsname%%
      \put(7025,2579){\rotatebox{30.00}{\makebox(0,0){\strut{}Naive}}}%
      \put(7025,2435){\rotatebox{30.00}{\makebox(0,0){\strut{} \texttt{tally}}}}%
      \csname LTb\endcsname%%
      \put(7224,2136){\makebox(0,0){\strut{}15.931s}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={396.00bp},height={170.00bp}]{timing}}%
    \gplfronttext
  \end{picture}%
\endgroup

